SAPIEN: A SimulAted Part-based Interactive ENvironment

Building home assistant robots has long been a pursuit for vision and robotics researchers. To achieve this task, a simulated environment with physically realistic simulation, sufficient articulated objects, and transferability to the real robot is indispensable. Existing environments achieve these requirements for robotics simulation with different levels of simplification and focus. We take one step further in constructing an environment that supports household tasks for training robot learning algorithm. Our work, SAPIEN, is a realistic and physics-rich simulated environment that hosts a large-scale set for articulated objects. Our SAPIEN enables various robotic vision and interaction tasks that require detailed part-level understanding.We evaluate state-of-the-art vision algorithms for part detection and motion attribute recognition as well as demonstrate robotic interaction tasks using heuristic approaches and reinforcement learning algorithms. We hope that our SAPIEN can open a lot of research directions yet to be explored, including learning cognition through interaction, part motion discovery, and construction of robotics-ready simulated game environment.

==> tex/data.tex <==
SAPIEN Asset is our simulation content, shown in the right box in Figure \ref{fig:sapien_diagram}. It contains robot models and the PartNet-Mobility dataset, which is our main contribution to simulatable robotics content.

\subsection{SAPIEN Assets}

\newcommand{\twoline}[2]{\begin{tabular}[c]{@{}c@{}}#1\\ #2\end{tabular}}
%\setlength{\tabcolsep}{3pt}

\begin{table*}[t]
%   \renewcommand\arraystretch{0.1}
  \centering
  \setlength{\tabcolsep}{1pt}
  \small
    \begin{tabular}{c|cccccccccccccccc}
    \toprule[2pt]
          & \small{\textbf{All}}   & \small{Bottle} & \small{Box}   & \small{Bucket} & \small{Cabinet} & \small{Camera} & \small{Cart}  & \small{Chair} & \small{Clock} & \twoline{\small{Coffee}}  & \twoline{\small{Dish}}{\small{Washer}} & \small{Dispenser} & \small{Door}  & \twoline{\small{EyeGls}} & \small{Fan}   & \small{Faucet} \\ \hline
    \#M   & \textbf{2,346} & 57    & 28    & 36    & 345   & 37    & 61    & 80    & 31    & 55    & 48    & 57    & 36    & 65    & 81    & 84 \\
    \#P   & \textbf{14,068} & 114   & 94    & 74    & 1,174 & 341   & 232   & 1,235 & 106   & 374   & 112   & 162   & 103   & 195   & 172   & 228 \\
    \midrule[1pt]
          & \twoline{\small{Chair?}}  & \small{Fridge} & \ll{Globe} & \small{Kettle} & \twoline{\small{Keybrd}} & \small{Knife} & \small{Lamp}  & \small{Laptop} & \small{Lighter} & \twoline{\small{Micro}} & \small{Monitor} & \small{Mouse} & \small{Oven}  & \small{Pen}   & \small{Phone} & \small{Pliers} \\
    \hline
    \#M   & 26    & 44    & 61    & 29    & 37    & 44    & 45    & 56    & 28    & 16    & 37    & 14    & 30    & 48    & 17    & 25 \\
    \#P   & 58    & 118   & 130   & 66    & 3,593 & 149   & 165   & 112   & 86    & 85    & 93    & 61    & 214   & 97    & 271   & 59 \\
    \midrule[1pt]
          & \small{Pot}   & \small{Printer} & \small{Remote} & \small{Safe}  & \small{Scissors} & \small{Stapler} & \twoline{\small{Suit-}}{\small{case}} & \small{Switch} & \small{Table} & \small{Toaster} & \small{Toilet} & \twoline{\small{Trash}}{\small{Can}} & \twoline{\small{USB}} & \twoline{\small{Washing}} {\small{Machine}} & \small{Window} &  \\
    \hline
    \#M   & 25    & 29    & 49    & 30    & 47    & 23    & 24    & 70    & 101   & 25    & 69    & 70    & 51    & 17    & 58    &  \\
    \#P   & 53    & 376   & 1,490 & 202   & 94    & 69    & 101   & 195   & 420   & 116   & 229   & 208   & 103   & 144   & 195   &  \\
    \bottomrule[2pt]
    \end{tabular}
  \label{tab:addlabel}
  \caption{\textbf{Statistics?????? of PartNet-Mobility Dataset}. \#M and \#P shows the number of models and movable parts respectively.}
  \vspace{-4mm}
\end{table*}

Our PartNet-Mobility dataset contains \textbf{2,346} object models from \textbf{46} categories. In total, there are \textbf{14,068} movable parts. All object categories are for indoor scenes collected from 3D Warehouse. We annotated 3 types of motions: hinge, slider, and screw, where hinge indicates rotation around an axis (doors); slider indicates translation along an axis (drawer), and screw indicates a combined hinge and slider (bottle cap, swivel chair). For hinge and slider joints, we annotate the motion limit (angles and lengths). For screw, we annotate the motion limits and whether the 2 degrees of freedom are coupled. Each joint has a parent and a child, and the collection of connected bodies and joints is called an articulation. We require the joints of an articulation to follow a tree structure with a single root, since most physical simulator handles tree-structured joint system well. Next, for each movable part, we assign a category-specific semantic label. We discuss the format of this dataset and the annotation efforts for extending PartNet~\cite{Mo_2019_CVPR} to the interaction-rich \textbf{PartNet-Mobility Dataset}.

\subsection{SAPIEN Asset Loader}
Unified Robot Description Format (URDF) is a common format for representing a physical model.  For each object in the SAPIEN Asset, including PartNet-Mobility models and robot models, we provide an associated URDF file, which can be loaded in simulation. For accurate simulation of contact, we decompose meshes into convex part using \cite{mamou2016volumetric, huang2018robust}.
Currently, we randomize or manually set the physical properties, e.g. friction, damping, density, to proper range. For robot models, we also provide C++/Python APIs to create a robot piece by piece to avoid complications introduced by URDF.


\subsection{Annotation Procedure}
This annotation procedure has 3 steps: enriching PartNet with more articulated objects, annotating part motions on PartNet models, post-processing to make them simulation-ready.

\paragraph{Enrich PartNet Models.} The PartNet dataset contains over 26K 3D models. However, most of them do not contain relative motions or clean textures. In the end, we select less than 1K PartNet models to include in our dataset. To enrich this dataset, we manually collected more models with part mobilities from 3D Warehouse \cite{3dwarehouse} and the ShapeNet dataset \cite{chang2015shapenet}. We then aligned the collected models to a consistent canonical pose and picked out the movable parts. \fanbo{unit sphere}

\paragraph{Annotating Part Motions.} We developed a web interface (Figure \ref{fig:annotation_interface}) for mobility annotation. This tool is a QA system, which proposes questions based on current stage of annotation. The questions are designed to minimize redundancy and exhaust all possible mobilities we have defined. 
% It exploits the hierarchical structures of PartNet to propose objects without relative mobility, and generates new questions based on past annotations. Using this tool, annotators will not miss any movable parts if they answer every question correctly. The output mobility annotations are guaranteed to satisfy tree properties suitable for simulation.\haozhu{refer to the new figure of annotation system here}

\begin{figure}
    \centering
    \includegraphics[width=.95\linewidth]{fig/annotation_interface.png}
    \caption{\textbf{Annotation interface.} 1) Part Tree: PartNet semantic tree that proposes fixed parts. 2) Motion tree: annotated movable parts. 3) Question: auto-generated exhaustive questions. 4) Visualization for current question and for motion axis annotation. }
    \label{fig:annotation_interface}
\end{figure}

% \begin{algorithm}
%     \caption*{\textbf{Building part motion tree}\haozhu{merge to Fig.4}}
%     \Minghua{Why the border lines are green?}
%     \begin{algorithmic}[1]
%         \For {There are parts can be fixed together}
%         \State Select a group of relatively fixed parts
%         \EndFor
%         \For {Hinge relationship exists}
%         \State Select parent and child
%         \State Pick the axis
%         \State Input motion range
%         \EndFor
%         \For {Slider relationship exists}
%         \State Select parent and child
%         \State Pick the axis
%         \State Input motion range
%         \EndFor
%         \State Determine other leaves
%     \end{algorithmic}
% \end{algorithm}

\paragraph{Post-processing.} In post processing, we double check the validity of the annotations, and then we determine semantic labels for each part in each category by first combining clues from our annotations and PartNet semantic trees. In the end, we produce a mobility dataset with clear motion parameters and part semantic labels. 

